HIRL: Hierarchical Inverse Reinforcement Learning for Long-Horizon Tasks with Delayed Rewards

Reinforcement Learning (RL) struggles in problems with delayed rewards, and one approach is to segment the task into sub-tasks with incremental rewards. We propose a framework called Hierarchical Inverse Reinforcement Learning (HIRL), which is a model for learning sub-task structure from demonstrations. HIRL decomposes the task into sub-tasks based on transitions that are consistent across demonstrations. These transitions are defined as changes in local linearity w.r.t to a kernel function. Then, HIRL uses the inferred structure to learn reward functions local to the sub-tasks but also handle any global dependencies such as sequentiality. We have evaluated HIRL on several standard RL benchmarks: Parallel Parking with noisy dynamics, Two-Link Pendulum, 2D Noisy Motion Planning, and a Pinball environment. In the parallel parking task, we find that rewards constructed with HIRL converge to a policy with an 80% success rate in 32% fewer time-steps than those constructed with Maximum Entropy Inverse RL (MaxEnt IRL), and with partial state observation, the policies learned with IRL fail to achieve this accuracy while HIRL still converges. We further find that that the rewards learned with HIRL are robust to environment noise where they can tolerate 1 stdev. of random perturbation in the poses in the environment obstacles while maintaining roughly the same convergence rate. We find that HIRL rewards can converge up-to 6x faster than rewards constructed with IRL.

==> 3-model-old.tex <==
\section{Sequential Consumable Rewards}\label{sec:seq}
We study tasks where trajectories are constructed from locally linear motions that switch upon receiving rewards.
The main challenge with segmentation is that it introduces sequential dependencies between the rewards.
Segmented rewards are consumable, that is only the agent's first visit to a goal state is rewarded, and conditioned on knowing which previous rewards were received.

\subsection{Sequential Consumable Rewards}
Let $[\rho_1, ...., \rho_k]$ define a sequence of $k$ regions of the state-space $\rho_i \subseteq S$. 
We call each of these $k$ regions a \emph{sub-goal}.
The agent starts at an initial state distribution $p_0$ with a current sub-goal of $\rho_1$. 
Upon reaching any state $s \in \rho_1$, the new sub-goal becomes $\rho_2$, and so on.
The reward achieved by the agent is the total number of sub-goals reached.
Thus, an optimal policy for such a reward is any policy $\pi$ such that the probability $k$ sub-goals are reached is maximized.
The key aspect of this model is that it enforces that the sub-goals are reached in the proper sequence.
To be able to learn such a reward function, we have to be able to infer $\{\rho_1,...,\rho_k\}$ from a set of demonstration trajectories $D$.
This will require a modeling assumption that rewards correlated with changes in agent motion, which is often the case in many physical tasks and Section \ref{sec:control} will provide more information.

It also turns out that such a reward structure is not compatible with the MDP $\mathcal{M}$ since it it has dependence on the past. To model this as a proper MDP, we have to use an MDP whose state-space also include history $\mathcal{M}_H$.
This definition is very useful in understanding the hardness of the general problem, and in Section \ref{sec:hard}, we show that the general problem is in fact computationally hard since identifying optimal features is equivalent to Non-Deterministic Finite Automata minimization.

\subsection{Demonstration Model}
We are given a set of demonstrations $D=\{d_1,...,d_N\}$ that are sequences of states and actions of an optimal policy.
Along with each $d_i$, let $\mathbf{x}_i(t)$ represents a trajectory in feature space $[\mathbf{x}_i(t)= f(s_1,a_1),...,f(s_T,a_T)]$.
We model the agent's trajectory in $\mathbb{R}^p$ as a sequence of variable length locally linear dynamical motions.
These motions are generated by an unknown switching linear dynamical system with zero-mean, normally distributed process noise:
\[
\mathbf{x}(t+1) = A_{i}\mathbf{x}(t) + W(t) \text{ : } A_i \in \{A_1,...,A_m\}.
\]
\emph{Transitions} are defined as times where $A(t) \ne A(t+1)$.
Thus, each transition will have an associated feature value $\mathbf{x}(t)$ called a transition state.
We model these $\mathbf{x}(t)$ as generated from a Gaussian Mixture Model over the feature space $\mathbb{R}^p$ and time (see Krishnan et al. for details~\cite{krishnan2015tsc}).
At first glance, the linearity assumption might seem quite strong, but it turns out that the demonstrations need to be linear in \emph{some} feature-space, which can be achieved with kernel dimensionality reduction (Section \ref{sec:kern}).
 
We interpret this mixture model as defining sub-goals for the task.
If there $k$ mixture components for the distribution $\{m_1,...,m_k\}$, the $\alpha$-quantile of each component distribution will define a region $\{\rho_1,...,\rho_k\}$ over the feature space at some time-interval.
We interpet the learned $\{\rho_1,...,\rho_k\}$ as the sub-goals.
As in the model, rewards for the intermediate goals are earned at the first entry into each region only if all previous regions have been rewarded.

\subsection{Problem Statements}
In this paper, we address the following problems:

\vspace{0.5em}

\noindent\textbf{Transition State Problem: } Given a set of demonstrations $D$ and a featurization $f$, identify $\{\rho_1,...,\rho_k\}$.

\vspace{0.5em}

\noindent\textbf{Segment Encoding Problem: } 
At any time $t$, let $H_t$ denote the sequence of previously visited states by an agent.
Using $\{\rho_1,...,\rho_k\}$, we construct a function $e(\cdot)$ that maps $H_t$ to a $k$-dimensional feature vector $v$ recording previously achieved sub-goals. 
We want to find a $k$-dimensional vector that most accurately represents the history of a process with $k$ transition states.

\vspace{0.5em}

\noindent\textbf{Reward Function Construction: }
We will use $v$ to construct reward functions for the sequential task.
We explore using quadratic distance-to-state rewards and integrating this vector with IRL.
$v$ will augment the state-space $S$, and we use Maximum Entropy Inverse Reinforcement Learning to learn a reward function across the feature space $\mathbb{R}^p$ and $v$. 
To use this reward function in Forward RL, the state-space is augmented with $v$.

==> 3-problemsetup.tex <==
%\documentclass[0-main.tex]{subfiles}
%\begin{document}

\section{Model Analysis}
In this section, we analyze the model and provide some formal interpretations.

\subsection{Sequence of Stable Feedback Controllers}\label{sec:control}
We have provided an informal justification of the locally-linear Transition State model in terms of object contacts and manipulation conditions.
Now, we formalize these conditions from a control theoretic perspective.
This model naturally follows from a system controlled with linear state feedback control to the centroids of $k$ target regions $[\rho_1,...,\rho_k]$. 

In the Transition State Model,  $[\rho_1,...,\rho_k]$ are defined as the superlevel sets of multivariate Gaussian distributions.
For each of the Gaussian mixture components, let $\{\mu_1,...,\mu_k\}$ denote the respective expectations and $\{\Sigma_1,...,\Sigma_k\}$ denote the respective covariances.
We can show that the Transition State Clustering model naturally follows from of a sequence of stable linear full-state feedback controllers sequentially controlling the system to each $\mu_i$ (up-to some tolerance defined by $\alpha$).

Suppose, we model the agent's trajectory in feature space as a linear dynamical system with a fixed dynamics.
Let $A_r$ model the agent's linear dynamics and $B_r$ model the agent's control matrix:
\[
\mathbf{x}(t+1) = A_r\mathbf{x}(t) + B_r\mathbf{u}(t) + W(t).
\]
For a particular mixture component $i$, the agent applies a linear feedback controller with gain $G_i$, regulating around the target state $\mu_i$.
This can be represented as the following system:
\[
\hat{\mathbf{x}}(t) = \mathbf{x}(t) - \mu_i 
\]
\[
\hat{\mathbf{x}}(t+1) = (A_r-G_iB_r)\hat{\mathbf{x}}(t)+ W(t).
\]
If this system is stable, it will converge to the state $\hat{\mathbf{x}}(t) = \mathbf{0}$ which is  $\mathbf{x}(t) = \mu_i$ as $t \rightarrow \infty$.
However, since this is a finite time problem, we model a stopping condition, namely, the system is close enough to $\mathbf{0}$.
For some $z_\alpha$ (e.g., in 1 dimension 95\% quantiles are $Z_{5\%} = 1.96$):
\[
\hat{\mathbf{x}}(t)^T \Sigma^{-1}_i \hat{\mathbf{x}}(t) \le z_\alpha.
\]
If the agent's trajectory was modeled as a sequence $1...K$ of such controllers, we would observe the Transition State Clustering model with each $A_i = A_r-G_iB_r$, and the clusters would be an Expectation Maximization estimate of the $(\mu_i, \Sigma_i)$.

\subsection{History MDP}
Strictly speaking, the model posed in the previous section is not an MDP since its reward function depends on the past.
To model this dependence on the past, we have to model an MDP whose state-space also include history.
At first glance, this may seem impractical, but we can show that leveraging the segmentation to compress this prior history leads to tractable learning problem.

Given a finite-horizon MDP $\mathcal{M}$ as defined in Section \ref{sec:back}, we can define an MDP $\mathcal{M}_H$ as follows.
Let $\mathcal{H}$ denote set of all dynamically feasible sequences of length $\le T$ comprised of the elements of $S$.
Therefore, for an agent at any time $t$, there is a sequence of previously visited states $H_t \in \mathcal{H}$.
The MDP $\mathcal{M}_H$ is defined as:
\[
\mathcal{M}_H = \langle S \times \mathcal{H},A,P'(\cdot,\cdot), R_\theta(\cdot,\cdot),T \rangle.
\]
For this MDP, $P'$ not only defines the transitions from the current state $s \mapsto s'$, but also increments the history sequence $H_{t+1} = H_{t} \sqcup s$.
Accordingly, the parametrized reward function $R_\theta$ is defined over $S$, $A$, and $H_{t+1}$.
In principle, one could apply IRL directly to $\mathcal{M}_H$.
However, we show that the general problem is computationally hard.

\vspace{0.5em}

\subsubsection{Representation Problem}
Consider the general case of the IRL problem, given $\mathcal{M}_H$ with an unknown reward function with arbitrary dependence on history and a set of demonstration trajectories $D$, infer the reward function $R$.

We want to understand the complexity of this general problem\footnote{Note that our analysis is done in the discrete case as typical with Reinforcement Learning,  but it is not a restriction of the method}.
First, it is clearly impractical to exactly represent $R$ in all but toy examples.
We quantify this by the dimensionality of the parameters needed to describe $R$, where in the worst case we need one parameter for each sequence in $\mathcal{H}$.

\vspace{0.5em}

\begin{proposition}[Space Complexity]
If $\mathcal{M}_H$ is a finite-state MDP, then the representation of $R$ for $\mathcal{M}_H$ has a worst-case parameter dimensionality of $\mathbf{O}(\exp(T))$.
\end{proposition}

\vspace{0.5em}

\subsubsection{Encoding Problem}
Instead, our model concisely encodes the history of the agent $H_t \in \mathcal{H}$ in terms of segments previously traversed which is a $k$ dimensional vector.
Then, additional complexity of representing the reward with history is $\mathbf{O}(k)$ instead of exponential.
We formalized a model where the rewards are sparse; a very small number of the possible sequences $\mathcal{H}_R \subseteq \mathcal{H}$ lead to non-zero rewards.

\todo{There is a commented out proof showing that feature selection for the general problem is PSPACE-Hard, SK is in the process of re-writing.}

\iffalse
However, it turns out that sparsity is not the only important property.
For the class of tasks formalized in the previous section, the rewards have a very particular dependence on history.
It turns out this is crucial to avoid a PSPACE-Hard feature selection problem.

Let us consider what would happen if this was not the case, namely, that the rewards could have a more complex dependence on the history.
We model this as a feature selection problem.
Let us assume that the rewards for $\mathcal{M}_H$ have the following linear parametrized structure:
\[
R(s,H_t,a) =  f(s,H_t,a)^T \theta.
\]
The objective of the feature selection problem is to construct a feature vector $f(s,H_t,a)$ such that the reward function is completely determined.
Suppose, there are a finite set of sequences $\mathcal{H}_R=\{H_R^{(1)},...,H_R^{(k)}\}$ that lead to a non-zero reward.
Then, $f(s,H_t,a)$ can be an indicator vector indicating whether $H_t$ matches any of the elements of $\mathcal{H}_R$, and $\theta = \mathbf{1}$.
If we have a system where we observe the reward at every state $s$, can we determine $\mathcal{H}_R$?

\begin{proposition}[Feature Selection]
Given a finite-state MDP 
Given a reward function $R$ that is history dependent, identifying a minimal set of features (in terms of cardinality) such that $R$ is completely determined at every state is PSPACE-Hard.
\end{proposition}














This analysis is quite pessimistic and makes no assumptions about the structure of $S$ or $A$, and in practice, we often make such simplifying assumptions.


One such assumption is to consider rewards with following structure:
\[
R(s,H_t,a) =  f(s,H_t,a)^T \theta
\]
where $f(s,H_t,a)$ is a feature vector that maps the states and action pairs to $\mathbb{R}^p$.
Then, even over the history, the dimensionality of the parametrized reward function is $\mathbf{O}(p)$ since it is parametrized by a $p$ dimensional vector.
However, designing such a feature vector in $\mathbb{R}^p$ is typically left to the user.

The next question is how hard is it to construct such a feature vector optimally (i.e., completely determines a reward functions).
We will show that solving this problem in general would imply a solution Non-Deterministic Finite Automaton (NFA) minimization, thus the complexity class of the optimal feature selection problem is PSPACE-hard, which is widely conjectured to be harder than PTIME.

\vspace{0.5em}



\vspace{0.5em}

We show that one-specific instance of the problem is equivalent to NFA minimization, thus proving the result by reduction.



Consider a specific representation for $R$ that is a reward that is earned only is a certain set of states have been previously traversed:
\[
R'(s,a) = R(s,a) \cdot [\Pi_{i=0}^k \mathbf{I}(s_{i} \in H_t)]
\]
for $\{s_1,...,s_k\}$ that are states in the state-space $s_i \subseteq S$, the function $\mathbf{I}(s_{i} \in H_t)$ indicates whether the state $s_i$ has been previously traversed, and $R(s,a)$ is a binary reward earned for the current state.
To completely determine this class of rewards with $k$ features, we have to know $\{s_1,...,s_k\}$, i.e., optimal feature selection.

A deterministic finite automaton (DFA) $\mathcal{A}$ is an MDP but with deterministic transitions.
However, we are interested in how the reward transitions as a function of the state.
Let $S_A$ be the state-space of $\mathcal{A}$, define another finite-automaton $\mathcal{A}^R$ which has the state-space $S_A \times \mathbb{Z}_2$.
In its state, $\mathcal{A}^R$ also keeps track of the cumulatively achieved reward function $R'$. 
Since $R'$ is dependent on history  $\mathcal{A}^R$ is not a DFA but a Non-Deterministic Finite Automaton.
The problem of feature selection, i.e., determining all of the state-visit indicator functions, is equivalent to finding a minimal state representation for $\mathcal{A}^R$; removing impossible states and merging states whose effect on the reward are indistinguishable.
Thus, the problem of optimal feature selection is equivalent to finding a minimal NFA representation of the process, which is known to be PSPACE-complete.

\vspace{0.5em}

For the general problem, we either have inefficiency in space in terms of representing a complex reward function or we have inefficiency in time-complexity in selecting features to encode the reward.
While the general problem is hard, there might be special cases where we can exploit the structure of the task.
For example, in physical tasks, we often know that such important features of history correlate with object contacts, changes in motion, and forces/torques applied.
\fi

\subsection{Benefits of Knowing Segments}
There are two ways in which we can apply the sequential consumable reward model.
First, there are tasks that are inherently sequential such as assembly.
For such tasks, there is a natural notion of sub-goals (i.e., the assembly of all of the components), and it is clear that a consumable reward model is required to learn optimal policies.
A similar argument is clear for problems with partial observation, where some important states are not seen.
Knowing previously traversed states can disambiguate optimal actions.
Segmentation is one way to concisely encode the process history to allow for history dependent policies.

On the other hand, we also consider ``segmented" tasks, where the tasks can be solved without sequential consumable rewards albeit slowly.
Surprisingly, we find that fitting a consumable reward model to such tasks actually leads to rewards that sometimes converge faster in forward RL (Section \ref{sec:exp})--even over techniques such as classical IRL, and we provide some intuition on why this can be the case.

\todo{SK: will illustrate each one of these cases}

\subsubsection{Simpler Local Policies} The additional segment features $v$ can also simplify policies leading to faster convergence. Consider the case, where the optimal policy is piecewise constant for each task segment. While this policy is easy to describe in terms of the features $v$, it may can be difficult to model in terms of the state-space $S$.

\subsubsection{Predictable Recovery} For more complex tasks, the agent will likely encounter states not seen in the set of demonstrations $D$, which will not be reflected in the reward function. In this case, the agent will explore until it arrives at known states and continue.
The additional features $v$ that track the segment progress encourage the agent to recover to the next sub-goal.
On the other hand, without the additional features IRL can miss sub-goals, leading to more unseen states in the future.
We find that when the number of demonstrations is relatively small (e.g, $5$) rewards constructed with \tsh (IRL with segment features) converges faster than IRL alone.

%The contribution of this work is to develop a state-representation for IRL and not the IRL technique itself. Therefore, we consider a prototypical IRL method as an example called Maximum Entropy Inverse Reinforcement Learning (MaxEnt-IRL)~\cite{DBLP:conf/aaai/ZiebartMBD08}.

%\end{document}

==> 4-clustering.tex <==
%\documentclass[0-main.tex]{subfiles}
%\begin{document}

\section{\tshfull}\label{sec:algo}
This section describes the \tsh algorithm, which has four steps: (1) featurization, (2) transition identification, (3) transition correspondence, and (4) vectorization.

\subsection{Step 1. Featurization}
The first step is to apply $f$ to every state-action pair in the demonstrations.
Every $d_i$ in $D$ is a sequence of $T$ state-action pairs:
\[
[(s_1,a_1),...,(s_T,a_T)]
\]
For each state-action pair, we apply the featurization $ f(s_1,a_1),...,f(s_T,a_T)$.
This gives us a $T$-step trajectory in the feature space $\mathbb{R}^p$ which we denote as $\mathbf{x}(t)$.
In this work, we assume that the featurization is given to us, and hope to explore using techniques such as Deep Learning in the future.

\subsection{Step 2. Identification}
This subsection is largely inspired from a model proposed in prior work~\cite{krishnan2015tsc}.
Each demonstration, $\mathbf{x}(t)$, is a trajectory in $\mathbb{R}^p$.
Suppose there was only one dynamical mode, then following from the Gaussian process noise assumption, this would be a linear regression problem:
\[
\arg\min_A \|A X_t - X_{t+1}\|
\]
where $X_t$ is a matrix where each column vector is $\mathbf{x}(t)$.
To extend this to set of $A$ matrices, Moldovan et al.~\cite{moldovan2013dirichlet} proves that fitting a Jointly Gaussian model to $w(t) = \binom{\mathbf{x}(t+1)}{\mathbf{x}(t)}$ is equivalent to Bayesian Linear Regression.
The intuition is that Gaussian random variables are stable under affine transformations, and applying a Mixture of Gaussians model (GMM) essentially applies locally linear regression.
If we map each $w(t)$ to its most likely mixture component, then we can find the co-linear states.
In typical GMM formulations, we have to select the number of mixture components $m$ before hand.
However, we can apply new results in Bayesian non-parameteric statistics and jointly solve for the component locations and the number of components with an algorithm called DP-GMM~\cite{kulis2011revisiting} with a soft prior over the number of clusters\footnote{We use the default settings in \url{https://pypi.python.org/pypi/dpcluster}}.

The identification procedure is summarized in Algorithm \ref{alg:tsh1}.
We construct a data matrix $W$ which is the set of $w(t)$ over all demonstrations and times.
We apply DP-GMM to $W$ and map each $w(t)$ to a most likely mixture component, and thus for each demonstration $i$ we get $w_{index}^{(i)}(t)$ which gives us the cluster index at time $t$.
Then, we identify all of the times $t$ such that $w_{index}^{(i)}(t) \ne w_{index}^{(i)}(t+1)$, and the final result is a set $\Theta$ of tuples of demonstration id $i$ and time $t$.

\subsection{Kernel Dimensionality Reduction}\label{sec:kern}
Transition identification makes an assumption about local-linearity.
However, we can relax this assumption by embedding the trajectories in a non-linear kernel space and identifying transitions in the embedded space.
Let $W = \{w_i\}$ be an indexed set of all $w(t)$ over all demonstration.
Let $\mathbf{\kappa}(w_0,w_1)$ define a kernel function over the set $W$.
For example, if $\mathbf{\kappa}$ is the radial basis function (RBF), then:
$ \mathbf{\kappa}(w_0,w_1) = e^{\frac{-\|w_0-w_1\|_2^2}{2\sigma}}$.
$\mathbf{\kappa}$ naturally defines a matrix $M$ where:
\[
M_{ij} = \mathbf{\kappa}(w_i,w_j) 
\]
The top $p'$ eigenvalues define a new embedded feature vector for each $w$ in $\mathbb{R}^{p'}$.
In this embedded space, we can apply our transition identification procedure.
This procedure allows us to model some types of non-linearities and states with different scaling properties.
In our experiments, we use an RBF kernel function in the cases where the feature-space dynamics were non-linear. 

\begin{algorithm}[t]
\small
\DontPrintSemicolon
\caption{Transition Identification \label{alg:tsh1}}
\KwData{Set of demonstrations:$\mathcal{D}$}

$W \leftarrow \emptyset$

\ForEach{$d_i \in \mathcal{D}$}{
   \ForEach{$t \in 0,1,...,T_i$}{
        $w(t) = \binom{\mathbf{x}(t+1)}{\mathbf{x}(t)}$
        
        $W = W \cup w(t)$
   }
}
$\{w_{index}^{(1)}(t),...,w_{index}^{(N)}(t)\} \leftarrow$ \texttt{DP-GMM(W)}
\vspace{0.5em}

$\Theta \leftarrow \emptyset$

\ForEach{$d_i \in \mathcal{D}$}{
   \ForEach{$t \in 0,1,...,T_i$}{
        \If{$w_{index}^{(i)}(t) \ne w_{index}^{(i)}(t+1)$}{
        $\Theta = \theta \cup (i,t)$
        }
   }
}

\KwResult{The set of transitions $\Theta$}
\end{algorithm}

\subsection{Step 3. Correspondence}
Across all demonstrations, the set of transition states induces a density over the feature-space and time.
Intuitively, when an agent enters certain regions of the state-space at certain times, there is a propensity to switch.
We are interested in aggregating nearby (spatially and temporally) transition states together.
We model this density as a Gaussian Mixture Model with $k$ mixture components $\{m_1,...,m_k\}$.
As before, we learn this with DP-GMM in the feature space to find these clusters.

Each of the mixture components is a multivariate Gaussian distribution with some mean and covariance.
Individually, each of the mixture components is a Gaussian distribution, and defines an $\alpha$-quantile region of the feature space and a time interval:
\[
G = \{\rho_1, \rho_2,...,\rho_m\}
\]
The overall procedure is summarized in Algorithm \ref{alg:tsh2}.

\begin{algorithm}[t]
\small
\DontPrintSemicolon
\caption{Transition State Clustering \label{alg:tsh2}}
\KwData{Set of transitions:$\Theta$}

$Y \leftarrow \emptyset$

\ForEach{$(i,t) \in \Theta$}{
   $Y \leftarrow Y \cup x^{(i)}(t)$
}
$G = \{\rho_1, \rho_2,...,\rho_m\}\leftarrow$ \texttt{DP-GMM(Y)}

\KwResult{The set of transition state clusters $G$}
\end{algorithm}

\subsection{Step 4. Vectorization}
Next, we show how to turn $G$ into a hash function $C_k$.
Suppose we have a trajectory of states $\mathbf{x}(t)$ from 0 to $T$.
This trajectory defines $T-1$ history vectors $H_2,...,H_T$ of all preceding states until time $T$.
For each $H_t$, we have our encoding function:
\[
e(H_t) = \sum_{i=1}^t C_k(s_i)
\]
Let $k$ be the number of GMM mixture components found by the procedure in the previous subsection.
For each $s_i$, we define an $k$ dimensional binary vector where component $j$ is 1: if $i$ is contained in the time interval $\tau_j$, the state $s_i$ is contained in $\rho_j$, and all previous components $1...j-1$ are 1. 
Thus, $e(H_t)$ the number of time-steps spent in each of the transition states conditioned on the event that all previous transition states are visited.
Algorithm \ref{alg:tsh3} summarizes this process.

\begin{algorithm}[t]
\small
\DontPrintSemicolon
\caption{Transition State Hashing \label{alg:tsh3}}
\KwData{Set of transition state clusters:$G$}
\KwData{Set of history states to hash:$H_t$}

$E \leftarrow [0,...,0]$

\ForEach{$(x,t) \in H_t$}{
   \If{$(x,t) \in$  \texttt{conf}(G)}{
      $i \leftarrow$ \texttt{find}(G,(x,t))
      
      $E[i] \leftarrow E[i] + 1$
   }
}

\KwResult{The hashed value of the history states $E$}
\end{algorithm}

%\end{document}

==> 9-dump.tex <==
\section{Latent State $H_t$}
\todo{****  THIS IS DUMP FILE *****}
Describe the process of linking kinematics and video (PCA, CCA, etc.).
If we apply any VLAD or encoding, or batching, describe it here:

\begin{itemize}
\item Encoding - Current Status
\begin{itemize}
\item So I've implemented the following encoding method- Latent Content Descriptors (LCD) + VLAD. However, initial results weren't great and I need to see how it performs on milestones clustering.
\end{itemize}


Vector of Locally Aggregated Descriptors (VLAD) image encoding as proposed by \cite{jegou2010aggregating} is a method a feature encoding and pooling method, similar to Fisher vectors. VLAD encodes a set of local feature descriptors $I=(x_1,\ldots,x_n)$ extracted from an image using a codebook $\mathrm{C} = \{c_1, \ldots, c_m \}$ built using a clustering method such as Gaussian Mixture Models (GMM) or K-means clustering.


VLAD was shown to perform better than Fisher vectors and average pooling for encoding multiple frames~\cite{xu2014discriminative}.

\item Temporal Batching - Current Status
\begin{itemize}
\item While batching is supposed to help in video analysis , I've seen good separation of clusters (PCA on conv features) with just individual frames without clustering... I think I need to look into this more and need to test it out with milestones clustering.
\end{itemize}

\end{itemize}



%%%% TABLE 1
                 & Z             &              &               & k+Z          &              &              \\ \hline
                 & CCA           & GRP          & PCA           & CCA          & GRP          & PCA          \\ \hline \hline
SIFT             &          -     &        -     & -0.113$\pm$0.016 & -            & -            & 0.284$\pm$0.122 \\ \hline
AlexNet conv3    & -0.013$\pm$0.012 & 0.117$\pm$0.035 & 0.200$\pm$0.024  & 0.272$\pm$0.112 & 0.281$\pm$0.119 & 0.267$\pm$0.120 \\ \hline
AlexNet conv4    & -0.025$\pm$0.009 & 0.135$\pm$0.013 & 0.213$\pm$0.007  & 0.294$\pm$0.114 & 0.277$\pm$0.134 & 0.273$\pm$0.102 \\ \hline
AlexNet pool5    & -0.029$\pm$0.023 & 0.129$\pm$0.016 & 0.197$\pm$0.009  & 0.281$\pm$0.134 & 0.258$\pm$0.102 & 0.276$\pm$0.128 \\ \hline
VGG conv5\_3     & -0.012$\pm$0.025 & 0.141$\pm$0.010 & \textbf{0.273$\pm$0.018}  & 0.247$\pm$0.099 & 0.287$\pm$0.138 & 0.325$\pm$0.113 \\ \hline
VGG LCDVLAD     & 0.046$\pm$0.020  & 0.012$\pm$0.002 & 0.068$\pm$0.023  & 0.294$\pm$0.088 & 0.331$\pm$0.088 & 0.224$\pm$0.056 \\ \hline
AlexNet LCD VLAD & 0.068$\pm$0.035  & 0.033$\pm$0.001 & -0.063$\pm$0.053 & 0.285$\pm$0.092 & 0.308$\pm$0.098 & 0.243$\pm$0.102 \\ 



% \begin{figure*}[t!]
%     \centering
%     \includegraphics[width=0.8\linewidth]{figures/suturing}
% 	\caption{Suturing: The figure shows a sequence of images for the Suturing in JIGSAWS dataset\cite{gao2014jigsaws}.
% The first row shows a manual segmentation of the task in 4 semantic steps: (1) Needle Positioning, (2) Needle Pushing, (3) Pulling Needle, (4) Hand-off.The task involves 4 repetitions of the 4-step cycle and runs for approx. 100s (frame numbers are at 30 fps). We show the sub-task level segmentation results from our completely unsupervised approach with only Kinematics data, only Visual data and a concatenation of both. The figure also shows (in magenta) frames of predicted Needle Hand-off, and (in orange) a new transition for needle re-orientation between needle push and needle pull.
% }
% 	\label{fig:suturing}
% 	\vspace{-5pt}
% \end{figure*}


\begin{table}[ht]
\centering
\caption{Comparison of \TSC performance on Suturing and Needle Passing Tasks. We compare the prediction performance by incrementally adding demonstrations from Experts~(E), Intermediates~(I), and Novices~(N) respectively to the dataset.\todo{Experiments running on machine}}
\label{tab:jigsaws}
\begin{tabular}{ll|l|l|l|l|l|l}
\multicolumn{2}{c}{}                                     &     \multicolumn{3}{c}{\cellcolor[HTML]{CBCEFB}Silhouette Score} & \multicolumn{3}{c}{\cellcolor[HTML]{FFC72C}DTW Score}\\
\multicolumn{2}{c}{}    & \multicolumn{1}{c|}{K} & \multicolumn{1}{c|}{Z} & \multicolumn{1}{c|}{K+Z}& \multicolumn{1}{c|}{K} & \multicolumn{1}{c|}{Z} & \multicolumn{1}{c}{K+Z} \\ \hline \hline 
\rowcolor[HTML]{E0E0E0}
\cellcolor[HTML]{CBCEFB}                                 & E     & &    &   &   &  &    \\ 
\cellcolor[HTML]{CBCEFB}                                 & E+I   & &    &   &   &  &    \\ 
\rowcolor[HTML]{E0E0E0}
\multirow{-3}{*}{\cellcolor[HTML]{CBCEFB}Suturing}       & E+I+N & &    &   &   &  &    \\ 
\cellcolor[HTML]{FFC72C}                                 & E     & &    &   &   &  &    \\ 
\rowcolor[HTML]{E0E0E0}
\cellcolor[HTML]{FFC72C}                                 & E+I   & &    &   &   &  &    \\ 
\multirow{-3}{*}{\cellcolor[HTML]{FFC72C}\parbox{1.2cm}{Needle Passing}} & E+I+N & &    &   &   &  &    \\ \hline
\end{tabular}
\end{table}


% \begin{figure}[t]
%     \centering
% 	\includegraphics[width=\linewidth]{figures/needle_passing}
% 	\caption{Needle Passing}
% 	\label{fig:needlePassing}
% 	\vspace{-5pt}
% \end{figure}


% ==============================================

% \begin{algorithm}[t]
% \caption{The Transition State Clustering Algorithm \todo{Fix with changes} \label{algotext}}
% % \begin{algorithmic}[1]
% \scriptsize
% \State \textsf{Input: } $\mathcal{D}$, $\rho$ pruning parameter, and $\delta$ compaction parameter.

% \State $n(t) = \binom{\mathbf{x}(t+1)}{\mathbf{x}(t)}$. 

% \State Cluster the vectors $n(t)$ using DP-GMM assigning each state to its most likely cluster. 

% \State \emph{Transition states} are times when $n(t)$ is in a different cluster than $n(t+1)$. 

% \State Remove states that transition to and from clusters with less than a fraction of $p$ demonstrations. 

% \State Remove consecutive transition states when the L2 distance between these transitions is less than $\delta$. 

% \State Cluster the remaining transition states in the state space $\mathbf{x}(t+1)$ using DP-GMM.

% \State Within each state-space cluster, sub-cluster the transition states temporally. 

% \State \textsf{Output: } A set $\mathcal{M}$ of clusters of transition states and the associated with each cluster a time interval of transition times.
% % \end{algorithmic}
% \end{algorithm}

        \resizebox{\linewidth}{!}{% put in textwidth
            \begin{tabular}{ll|l|l|l|l|l|l}
            \multicolumn{2}{c}{}                                     &     \multicolumn{3}{c}{\cellcolor[HTML]{CBCEFB}Silhouette Score} & \multicolumn{3}{c}{\cellcolor[HTML]{FFC72C}DTW Score}\\
            \multicolumn{2}{c}{}    & \multicolumn{1}{c|}{K} & \multicolumn{1}{c|}{Z} & \multicolumn{1}{c|}{K+Z}& \multicolumn{1}{c|}{K} & \multicolumn{1}{c|}{Z} & \multicolumn{1}{c}{K+Z} \\ \hline \hline 
            \rowcolor[HTML]{E0E0E0}
            \cellcolor[HTML]{CBCEFB}                                 & E     & &    &   &   &  &    \\ 
            \cellcolor[HTML]{CBCEFB}                                 & E+I   & &    &   &   &  &    \\ 
            \rowcolor[HTML]{E0E0E0}
            \multirow{-3}{*}{\cellcolor[HTML]{CBCEFB}Suturing}       & E+I+N & &    &   &   &  &    \\ 
            \cellcolor[HTML]{FFC72C}                                 & E     & &    &   &   &  &    \\ 
            \rowcolor[HTML]{E0E0E0}
            \cellcolor[HTML]{FFC72C}                                 & E+I   & &    &   &   &  &    \\ 
            \multirow{-3}{*}{\cellcolor[HTML]{FFC72C}\parbox{1.2cm}{Needle Passing}} & E+I+N & &    &   &   &  &    \\ \hline
            \end{tabular}
        }
        
        
        \begin{tabular}{ll|l|l|l}
        \hline
        \multicolumn{2}{c}{\cellcolor[HTML]{CBCEFB} Toy Example}  & \multicolumn{1}{c|}{\parbox{1.5cm}{Target Noise}} & \multicolumn{1}{c|}{\parbox{1.5cm}{Control Noise}} & \multicolumn{1}{c}{\parbox{2cm}{Kinematics\\ Sensor Noise}} \\ \hline \hline 
        \rowcolor[HTML]{E0E0E0}
        \cellcolor[HTML]{CBCEFB}                                 & K     & &    &   \\ 
        \cellcolor[HTML]{CBCEFB}                                 & Z   & &    &     \\ 
        \rowcolor[HTML]{E0E0E0}
        \multirow{-3}{*}{\cellcolor[HTML]{CBCEFB}\parbox{1.3cm}{Silhouette Score}}       & K+Z & &     &  \\ 
        \cellcolor[HTML]{FFC72C}                                 & K     & &    &   \\ 
        \rowcolor[HTML]{E0E0E0}
        \cellcolor[HTML]{FFC72C}                                 & Z   & &    &     \\ 
        \multirow{-3}{*}{\cellcolor[HTML]{FFC72C}\parbox{1.3cm}{DTW Score}} & K+Z & &    &    \\ \hline
        \end{tabular}
        
        
        
\iffalse
\subsubsection{Evaluation of Results }

\noindent \textit{Exp1. End-to-end result with some task}

\begin{enumerate}
\item Show that clusters are sensible and align with some intuitive criteria e.g., surgemes
\end{enumerate}

\noindent \textit{Exp2. Does Vision Help}

\begin{enumerate}
\item Remove visual features and show that clusters degrade
\end{enumerate}

\noindent \textit{Exp3. Parameter Search}

\begin{enumerate}
\item Describe our eval procedure and how we arrived at the architecture we did.
\end{enumerate}

\noindent \textit{Robustness}
\begin{enumerate}
\item Add noise or corrupt images and test to see how robust the segmentations we learn are.
\end{enumerate}
\fi

\iffalse
\subsection{Discussion}
\begin{enumerate}
\item How successful was our unsupervised approach in learning meaningful segmentations
\item RGB videos vs. RGB-D videos
\end{enumerate}
\fi

